SurCo: Learning Linear Surrogates For Combinatorial Nonlinear Optimization Problems

Optimization problems with nonlinear cost functions and combinatorial constraints appear in many real-world applications but remain challenging to solve efficiently compared to their linear counterparts. To bridge this gap, we propose $\textbf{SurCo}$ that learns linear $\underline{\text{Sur}}$rogate costs which can be used in existing $\underline{\text{Co}}$mbinatorial solvers to output good solutions to the original nonlinear combinatorial optimization problem. The surrogate costs are learned end-to-end with nonlinear loss by differentiating through the linear surrogate solver, combining the flexibility of gradient-based methods with the structure of linear combinatorial optimization. We propose three $\texttt{SurCo}$ variants: $\texttt{SurCo}-\texttt{zero}$ for individual nonlinear problems, $\texttt{SurCo}-\texttt{prior}$ for problem distributions, and $\texttt{SurCo}-\texttt{hybrid}$ to combine both distribution and problem-specific information. We give theoretical intuition motivating $\texttt{SurCo}$, and evaluate it empirically. Experiments show that $\texttt{SurCo}$ finds better solutions faster than state-of-the-art and domain expert approaches in real-world optimization problems such as embedding table sharding, inverse photonic design, and nonlinear route planning.

==> 000_notes.tex <==
Q: need words for different components of the pipeline:
1 features -> 2 coefficients -> 3 linear opt problem -> 4 solution -> 5 nonlinear objective (optionally fine-tuning)


surrogate: linear objective cTx
surrogate's optimization problem: min cTx s.t. x in X
{learned,heuristic,etc} algorithm: [1,4]
coefficient predictor: [1,2]


[5]: loss, global nonlinear objective, global loss <- if loss need to change to min, also maybe need to change to gradient descent

note: problems are in min formulation

TODO: determine orderings
predicted linear surrogate objective
vs
surrogate linear problem?

==> 01_introduction_old.tex <==

For instance, with the recent rise in deep learning, many people are interested in problems that consider training a neural network that estimates the value of a combinatorial solution, and then searching the feasible region for a solution that optimizes the solution quality as estimated by the neural network \cite{zha2022autoshard}.
\amf{citation needed for training nn then optimizing using nn as loss estimator, frank paper, any others? Should we reference stuff about optimizing gaussian processes or other nonlinear functions? Maybe something with combinatorial bandits} 
Similarly, several physically-constrained domains require solving a domain-specific nonlinear design problem with constraints enforcing that the design be physically viable, manufacturable with available tools, or being symmetric \cite{schubert_inverse_2022}.
\amf{Martin paper and possibly others?}
% limitations of current approaches
Solution approaches in these nonlinear combinatorial domains are generally comprised of heuristics that depend on the nature of the objective and feasible region. For instance, if the feasible region is simply selecting a subset of items that meet a budget, then one might consider greedy algorithms which iteratively select a single item at a time until the budget is reached. Similarly, when the problem considers allocating items to budget-constrained bins, a solver may iteratively make a single item-bin assignment at a time until the respective budgets are reached. In the case of ensuring physical manufacturability, solvers may maintain feasible solutions and make local modifications that preserve these desirable properties. 
% hope from linear optimization: it's fast
In many of these cases, there are a wide variety of practical and heavily tuned solvers for optimizing a linear function over the feasible region such as Mixed Integer Linear Programming (MILP) or greedy search among others. However, reducing the nonlinear optimization problem to an instance of integer linear optimization is often untenable without the help of an optimization specialist who can leverage domain knowledge. However, if we could effectively reduce the original combinatorial nonlinear optimization problem to a combinatorial linear optimization problem, then we could leverage the wide variety of high performance solvers and quickly generate high quality solutions. We do not necessarily want to model the entire nonlinear objective using a linear function, but rather we want to determine what linear objective will yield an optimal solution which has high quality for the original nonlinear objective. In order to generate this linear function, we consider that the original problem has high-level features describing the original nonlinear objective, the feasible region, and external data that may help construct the linear function. 
% snippet about benefit of training for a distribution.
Furthermore, many industrial settings face distributions of problem instances where the overall structure of the problem remains the same, but slightly different instances need to be solved on a regular basis with small variations in the nonlinear objective function or the combinatorial search space. As a result, we can leverage historical problem instances from the given distribution and pay the upfront cost of training on these historical problem instances so that we can quickly obtain high quality solutions on unseen problem instances.

% contributions
To tackle solving distributions of nonlinear combinatorial optimization problems we propose a method that trains a machine learning model to predict a linear surrogate objective based on high-level features of the original nonlinear problem. We leverage recent work in the area of differentiable optimization which computes gradients of the optimal solution of a linear combinatorial optimization problem with respect to linear objective coefficients \cite{poganvcic2019diffbb,niepert2021imle,berthet2020diffperturb}, so that we can effectively update the coefficients of the linear surrogate objective such that its solution has high quality when evaluated with the global nonlinear objective which acts as a loss. We focus on nonlinear combinatorial problems where the nonlinear objective is differentiable with respect to the solution and where the combinatorial feasible region can be efficiently searched over using standard techniques such as MILP or greedy search. Globally, we consider training a pipeline that takes in problem instance data, feeds it through a neural network that predicts surrogate linear objective coefficients which are then used to search the combinatorial feasible region for a solution optimizing those linear coefficients. The loss of the solution is computed via the differentiable nonlinear function and we backpropagate this loss through the surrogate linear optimization problem to the predicted coefficients and ultimately to the predictive network whose parameters we update. Thus, we train the full pipeline with gradient descent to produce high quality linear surrogates for solving unseen nonlinear optimization problems.


==> dlrm_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}
\begin{tabular}{@{}ccr@{}}
\toprule
\multicolumn{2}{c}{Table Placement}          &               \\ \midrule
Setting                  & Method            & Solution Quality (Latency) & Test Runtime \\ \midrule
\multirow{3}{*}{DLRM-10} & Greedy (on the fly)            & 8.9$\pm$0.0   \\
                         & DreamShard (offline)        & 7.7$\pm$0.3   \\
                         & Diff Opt Learned Surrogate (ours) & 4.8$\pm$0.3   \\ \midrule
\multirow{3}{*}{DLRM-20} & Greedy            & 12.6$\pm$0.0  \\
                         & DreamShard        & 11.6$\pm$0.2  \\
                         & Learned Surrogate & 5.5$\pm$0.3   \\ \midrule
\multirow{3}{*}{DLRM-30} & Greedy            & 13.1$\pm$0.0  \\
                         & DreamShard        & 13.1$\pm$0.2  \\
                         & Learned Surrogate & 8.1$\pm$0.5   \\ \midrule
\multirow{3}{*}{DLRM-40} & Greedy            & 21.8$\pm$0.1  \\
                         & DreamShard        & 19.9$\pm$0.3  \\
                         & Learned Surrogate & 11.9$\pm$0.7  \\ \midrule
\multirow{3}{*}{DLRM-50} & Greedy            & 37.4$\pm$0.1  \\
                         & DreamShard        & 35.5$\pm$0.7  \\
                         & Learned Surrogate & 25.4$\pm$0.9  \\ \midrule
\multirow{3}{*}{DLRM-60} & Greedy            & 48.7$\pm$0.1  \\
                         & DreamShard        & 49.6$\pm$0.8  \\
                         & Learned Surrogate & 35.9$\pm$0.9  \\ \bottomrule
\end{tabular}


\label{tab:results_dlrm}
\end{table}



==> photonics_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}ccrr@{}}
\toprule
\multicolumn{2}{l}{Inverse Photonics}                            &            &                        \\ \midrule
Setting                         & Method                         & Solution Quality (Success \%) & Deployment Runtime (s) \\ \midrule
\multirow{4}{*}{Bend}           & Pass-Through On-The-Fly        & 100\%      & 106                    \\
                                & Diff Opt On-The-Fly (ours)           & 100\%      & 41                     \\
                                & Pass-Through Learned Surrogate & 28\%       & 1.9                    \\
                                & Diff Opt Learned Surrogate (ours)     & 92\%       & 1.9                    \\ \midrule
\multirow{4}{*}{Demultiplexer}  & Pass-Through On-The-Fly        & 84\%       & 686                    \\
                                & Diff Opt On-The-Fly            & 92\%       & 593                    \\
                                & Pass-Through Learned Surrogate & 4\%        & 5.5                    \\
                                & Diff Opt Learned Surrogate     & 84\%       & 5.5                    \\ \midrule
\multirow{4}{*}{Mode Converter} & Pass-Through On-The-Fly        & 100\%      & 91                     \\
                                & Diff Opt On-The-Fly            & 100\%      & 33                     \\
                                & Pass-Through Learned Surrogate & 32\%       & 1.9                    \\
                                & Diff Opt Learned Surrogate     & 92\%       & 1.9                    \\ \midrule
\multirow{4}{*}{Beam Splitter}  & Pass-Through On-The-Fly        & 56\%       & 640                    \\
                                & Diff Opt On-The-Fly            & 68\%       & 575                    \\
                                & Pass-Through Learned Surrogate & 4\%        & 3.5                    \\
                                & Diff Opt Learned Surrogate     & 52\%       & 3.5                    \\ \bottomrule
\end{tabular}
\label{tab:results_photonics}
\caption{Results on inverse photonics settings both for optimizing on-the-fly using gradient-based update of latent cost parameters as well as training a model that predicts surrogate coefficients offline on a training dataset consisting of random training instances of the different problem settings. When training on-the-fly, we can either update the latent cost parameters using pass-through gradients as was done in previous work \cite{schubert_inverse_2022}, or use the proposed method which considers differentiating the solution of the optimizer with respect to the input objective coefficients. Additionally, we evaluate both approaches for obtaining gradients in the offline training setting where we train a model to predict latent coefficients for the optimization algorithm offline and then at test time run the brush algorithm with the predicted coefficients. We evaluate the number of test instances which are successfully solved to optimality with a loss of 0, as well as the deployment runtime of the different approaches. }
\end{table}
